Tree of Clarifications: Answering Ambiguous Questions with Retrieval-Augmented Large Language Models

Questions in open-domain question answering are often ambiguous, allowing multiple interpretations. One approach to handling them is to identify all possible interpretations of the ambiguous question (AQ) and to generate a long-form answer addressing them all, as suggested by Stelmakh et al., (2022). While it provides a comprehensive response without bothering the user for clarification, considering multiple dimensions of ambiguity and gathering corresponding knowledge remains a challenge. To cope with the challenge, we propose a novel framework, Tree of Clarifications (ToC): It recursively constructs a tree of disambiguations for the AQ -- via few-shot prompting leveraging external knowledge -- and uses it to generate a long-form answer. ToC outperforms existing baselines on ASQA in a few-shot setup across the metrics, while surpassing fully-supervised baselines trained on the whole training set in terms of Disambig-F1 and Disambig-ROUGE. Code is available at https://github.com/gankim/tree-of-clarifications.

==> tables/asqa_old.tex <==
\begin{table}[t!]
    % \small
    \centering
    \begin{threeparttable}
    % \setlength{\tabcolsep}{0.5em}
    \begin{tabular*}{0.98\columnwidth}{lccc}
        \toprule
        % \textbf{Model} & \multicolumn{3}{c}{OR-QuAC} \\
        \textbf{Model} & \textbf{D-F1} & \textbf{R-L}  & \textbf{DR} \\
        \midrule \midrule
        % \multicolumn{5}{c}{\textit{Upperbounds}} \\
        % \midrule
        % Human Performance & 64.8 & 49.4 & 98.4 & 61.8 \\
        % \midrule
        \multicolumn{4}{c}{\textit{Fully-supervised}} \\
        \midrule
        Fine-tuned T5-Large \\
        \quad Closed Book & 7.4 & 33.5 & 15.7 \\
        \quad w/ JPR & 26.4 & 43.0 &   33.7 \\
        Soft-Prompt Tuning \\
        \quad PaLM 540B & 27.8 & 37.4 & 32.1 \\
        \midrule
        \multicolumn{4}{c}{\textit{Few-shot Prompting (5-shot)}} \\
        \midrule
        \citet{amplayo2022query} \\
        \quad PaLM 540B & 25.3 & 34.5 & 29.6 \\
        \quad GPT-3 175B & 25.0 & 31.8 & 28.2 \\
        \midrule
        \textit{Ours} (GPT-3 175B) \\
        % \quad Depth = 0 & 30.8 & 36.0 & 29.4 & 32.5  \\
        \quad + RAC & 31.1 & 39.6 & 35.1  \\
        \quad \quad + \textsc{ToC} w/ BFS & 32.4 & \textbf{40.0} & 36.0  \\
        \quad \quad + \textsc{ToC} w/ Pruning & \textbf{33.7} & 39.7 & \textbf{36.6}  \\
        % \quad w/ Pruning & 82.1 & 40.6 & 31.8 & 36.0  \\
        % \quad + Pruning & - & - & - & -  \\
        
        \midrule
        \bottomrule
    \end{tabular*}
    \end{threeparttable}
    \caption{Comparison over fully-supervised and few-shot prompting baselines. We report evaluation results on the development set of ASQA~\cite{stelmakh-etal-2022-asqa}.
    }
    \label{table:main}
\end{table}
